Topological degree as a discrete diagnostic for disentanglement, with applications to the $\Delta$VAE

We investigate the ability of Diffusion Variational Autoencoder ($\Delta$VAE) with unit sphere $\mathcal{S}^2$ as latent space to capture topological and geometrical structure and disentangle latent factors in datasets. For this, we introduce a new diagnostic of disentanglement: namely the topological degree of the encoder, which is a map from the data manifold to the latent space. By using tools from homology theory, we derive and implement an algorithm that computes this degree. We use the algorithm to compute the degree of the encoder of models that result from the training procedure. Our experimental results show that the $\Delta$VAE achieves relatively small LSBD scores, and that regardless of the degree after initialization, the degree of the encoder after training becomes $-1$ or $+1$, which implies that the resulting encoder is at least homotopic to a homeomorphism.

==> reference.tex <==
@article{milnor1965topology,
  title={Topology from the differentiable viewpoint, Univ},
  author={Milnor, John},
  journal={Press of Virginia, Charlottesville},
  volume={1990},
  year={1965}
}

@book{hatcher2005algebraic,
  title={Algebraic topology},
  author={Hatcher, Allen},
  year={2005},
  publisher={Cambridge University Press}
}
  %publisher={清华大学出版社有限公司}


@inproceedings{kingma2013auto,
  author       = {Diederik P. Kingma and
                  Max Welling},
  editor       = {Yoshua Bengio and
                  Yann LeCun},
  title        = {Auto-Encoding {V}ariational {B}ayes},
  booktitle    = {2nd International Conference on Learning Representations, {ICLR} 2014,
                  Banff, AB, Canada, April 14-16, 2014, Conference Track Proceedings},
  year         = {2014},
  url          = {http://arxiv.org/abs/1312.6114},
  timestamp    = {Thu, 04 Apr 2019 13:20:07 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/KingmaW13.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@article{bengio2013representation,
  title={Representation learning: A review and new perspectives},
  author={Bengio, Yoshua and Courville, Aaron and Vincent, Pascal},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={35},
  number={8},
  pages={1798--1828},
  year={2013},
  publisher={IEEE}
}

@article{burgess2018understanding,
  title={Understanding disentangling in beta-{VAE}},
  author={Burgess, Christopher P and Higgins, Irina and Pal, Arka and Matthey, Loic and Watters, Nick and Desjardins, Guillaume and Lerchner, Alexander},
  journal={Learning Disentangled Representations: from Perception to Control Workshop, 2017},
  year={2017}
}


@article{higgins2018towards,
  title={Towards a definition of disentangled representations},
  author={Higgins, Irina and Amos, David and Pfau, David and Racaniere, Sebastien and Matthey, Loic and Rezende, Danilo and Lerchner, Alexander},
  journal={arXiv preprint arXiv:1812.02230},
  year={2018}
}

@inproceedings{cha2023orthogonality,
  title={Orthogonality-enforced latent space in autoencoders: an approach to learning disentangled representations},
  author={Cha, Jaehoon and Thiyagalingam, Jeyan},
  booktitle={International Conference on Machine Learning},
  pages={3913--3948},
  year={2023},
  organization={PMLR}
}

@inproceedings{kim2018disentangling,
  title={Disentangling by factorising},
  author={Kim, Hyunjik and Mnih, Andriy},
  booktitle={International conference on machine learning},
  pages={2649--2658},
  year={2018},
  organization={PMLR}
}

@article{davidson2018hyperspherical,
  title={Hyperspherical Variational Auto-Encoders},
  author={Davidson, Tim R. and
          Falorsi, Luca and 
          De Cao, Nicola and
          Kipf, Thomas and
          Tomczak, Jakub M.},
  journal={34th Conference on Uncertainty in Artificial Intelligence (UAI-18)},
  year={2018}
}


@article{falorsi2018explorations,
  title={Explorations in homeomorphic variational auto-encoding},
  author={Falorsi, Luca and De Haan, Pim and Davidson, Tim R and De Cao, Nicola and Weiler, Maurice and Forr{\'e}, Patrick and Cohen, Taco S},
  journal={ICML18 Workshop on Theoretical Foundations and Applications of Deep Generative Models},
  year={2018}
}


@inproceedings{ijcai2020p375,
  title     = {Diffusion Variational Autoencoders},
  author    = {Perez Rey, Luis A. and Menkovski, Vlado and Portegies, Jim},
  booktitle = {Proceedings of the Twenty-Ninth International Joint Conference on
               Artificial Intelligence, {IJCAI-20}},
  publisher = {International Joint Conferences on Artificial Intelligence Organization},
  editor    = {Christian Bessiere},
  pages     = {2704--2710},
  year      = {2020},
  month     = {7},
  note      = {Main track},
  doi       = {10.24963/ijcai.2020/375},
  url       = {https://doi.org/10.24963/ijcai.2020/375},
}


@article{esmaeili2024topological,
  title={Topological Obstructions and How to Avoid Them},
  author={Esmaeili, Babak and Walters, Robin and Zimmermann, Heiko and van de Meent, Jan-Willem},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

@article{menkovski2024small,
  title={Small time asymptotics of the entropy of the heat kernel on a Riemannian manifold},
  author={Menkovski, Vlado and Portegies, Jacobus W and Ravelonanosy, Mahefa Ratsisetraina},
  journal={Applied and Computational Harmonic Analysis},
  pages={101642},
  year={2024},
  publisher={Elsevier}
}

@inproceedings{tonnaer2022quantifying,
  title={Quantifying and Learning Linear Symmetry-Based Disentanglement},
  author={Tonnaer, Loek and Rey, Luis Armando Perez and Menkovski, Vlado and Holenderski, Mike and Portegies, Jim},
  booktitle={International Conference on Machine Learning},
  pages={21584--21608},
  year={2022},
  organization={PMLR}
}


@inproceedings{rezende2014stochastic,
  title={Stochastic backpropagation and approximate inference in deep generative models},
  author={Rezende, Danilo Jimenez and Mohamed, Shakir and Wierstra, Daan},
  booktitle={International conference on machine learning},
  pages={1278--1286},
  year={2014},
  organization={PMLR}
}

@article{chadebec2022data,
  title={Data augmentation in high dimensional low sample size setting using a geometry-based variational autoencoder},
  author={Chadebec, Cl{\'e}ment and Thibeau-Sutre, Elina and Burgos, Ninon and Allassonni{\`e}re, St{\'e}phanie},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={45},
  number={3},
  pages={2879--2896},
  year={2022},
  publisher={IEEE}
}


@article{de2018topological,
  title={Topological constraints on homeomorphic auto-encoding},
  author={de Haan, Pim and Falorsi, Luca},
  journal={NeurIPS 2018 workshop on Integration of Deep Learning Theories},
  year={2018}
}

@article{blanco1997evaluation,
  title={Evaluation of the rotation matrices in the basis of real spherical harmonics},
  author={Blanco, Miguel A and Fl{\'o}rez, Manuel and Bermejo, Margarita},
  journal={Journal of Molecular structure: THEOCHEM},
  volume={419},
  number={1-3},
  pages={19--27},
  year={1997},
  publisher={Elsevier}
}



@article{brocker2013representations,
  title={Representations of Compact Lie Groups},
  author={Br{\"o}cker, Theodor and tom Dieck, Tammo},
  journal={Graduate Texts in Mathematics},
  year={1985},
  publisher={Springer Berlin Heidelberg}
}


@article{caselles2019symmetry,
  title={Symmetry-based disentangled representation learning requires interaction with environments},
  author={Caselles-Dupr{\'e}, Hugo and Garcia Ortiz, Michael and Filliat, David},
  journal={Advances in Neural Information Processing Systems},
  volume={32},
  year={2019}
}

@article{alet2021noether,
  title={Noether networks: meta-learning useful conserved quantities},
  author={Alet, Ferran and Doblar, Dylan and Zhou, Allan and Tenenbaum, Josh and Kawaguchi, Kenji and Finn, Chelsea},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={16384--16397},
  year={2021}
}

@inproceedings{ding2020guided,
  title={Guided variational autoencoder for disentanglement learning},
  author={Ding, Zheng and Xu, Yifan and Xu, Weijian and Parmar, Gaurav and Yang, Yang and Welling, Max and Tu, Zhuowen},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={7920--7929},
  year={2020}
}

@article{huh2024isometric,
  title={Isometric Quotient Variational Auto-Encoders for Structure-Preserving Representation Learning},
  author={Huh, In and Choe, Jae Myung and KIM, YOUNGGU and Kim, Daesin and others},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

@article{carbonneau2022measuring,
  title={Measuring disentanglement: A review of metrics},
  author={Carbonneau, Marc-Andr{\'e} and Zaidi, Julian and Boilard, Jonathan and Gagnon, Ghyslain},
  journal={IEEE transactions on neural networks and learning systems},
  year={2022},
  publisher={IEEE}
}

@article{harmonicsclaus,
  title={Claus MUlier},
  author={Harmonics, Spherical},
  journal={Lecture Notes in Mathematics (LNM))},
  publisher={Springer},
  volume={17},
  year={1966}
}

@article{do2019theory,
  title={Theory and evaluation metrics for learning disentangled representations},
  author={Do, Kien and Tran, Truyen},
  journal={International Conference on Learning Representations, {ICLR} 2020},
  year={2020}
}

@article{van2019disentangled,
  title={Are disentangled representations helpful for abstract visual reasoning?},
  author={Van Steenkiste, Sjoerd and Locatello, Francesco and Schmidhuber, J{\"u}rgen and Bachem, Olivier},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@inproceedings{hoffman2016elbo,
  title={Elbo surgery: yet another way to carve up the variational evidence lower bound},
  author={Hoffman, Matthew D and Johnson, Matthew J},
  booktitle={Workshop in Advances in Approximate Bayesian Inference, NIPS},
  volume={1},
  year={2016}
}

@inproceedings{tomczak2018vae,
  title={VAE with a VampPrior},
  author={Tomczak, Jakub and Welling, Max},
  booktitle={International conference on artificial intelligence and statistics},
  pages={1214--1223},
  year={2018},
  organization={PMLR}
}

@article{sonderby2016ladder,
  title={Ladder variational autoencoders},
  author={S{\o}nderby, Casper Kaae and Raiko, Tapani and Maal{\o}e, Lars and S{\o}nderby, S{\o}ren Kaae and Winther, Ole},
  journal={Advances in neural information processing systems},
  volume={29},
  year={2016}
}

@article{klushyn2019learning,
  title={Learning hierarchical priors in vaes},
  author={Klushyn, Alexej and Chen, Nutan and Kurle, Richard and Cseke, Botond and van der Smagt, Patrick},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}


@article{liu2020metrics,
  title={Metrics for exposing the biases of content-style disentanglement},
  author={Liu, Xiao and Thermos, Spyridon and Valvano, Gabriele and Chartsias, Agisilaos and O’Neil, Alison and Tsaftaris, Sotirios A},
  journal={arXiv preprint arXiv:2008.12378},
  volume={7},
  year={2020}
}

@article{higgins2017beta,
  title={beta-{VAE}: Learning basic visual concepts with a constrained variational framework.},
  author={Higgins, Irina and Matthey, Loic and Pal, Arka and Burgess, Christopher P and Glorot, Xavier and Botvinick, Matthew M and Mohamed, Shakir and Lerchner, Alexander},
  journal={ICLR (Poster)},
  volume={3},
  year={2017}
}

@inproceedings{suter2019robustly,
  title={Robustly disentangled causal mechanisms: Validating deep representations for interventional robustness},
  author={Suter, Raphael and Miladinovic, Djordje and Sch{\"o}lkopf, Bernhard and Bauer, Stefan},
  booktitle={International Conference on Machine Learning},
  pages={6056--6065},
  year={2019},
  organization={PMLR}
}


@inproceedings{locatello2019challenging,
  title={Challenging common assumptions in the unsupervised learning of disentangled representations},
  author={Locatello, Francesco and Bauer, Stefan and Lucic, Mario and Raetsch, Gunnar and Gelly, Sylvain and Sch{\"o}lkopf, Bernhard and Bachem, Olivier},
  booktitle={international conference on machine learning},
  pages={4114--4124},
  year={2019},
  organization={PMLR}
}

@inproceedings{sepliarskaia2019not,
author = {Sepliarskaia, Anna and Kiseleva, Julia and de Rijke, Maarten},
booktitle = {ICML Workshop on Theoretic Foundation, Criticism, and Application Trend of Explainable AI},
date-added = {2021-06-18 07:13:54 +0200},
date-modified = {2021-06-24 21:13:49 +0200},
month = {July},
title = {How Not to Measure Disentanglement},
year = {2021}}


@inproceedings{szegedy2013intriguing,
  author       = {Christian Szegedy and
                  Wojciech Zaremba and
                  Ilya Sutskever and
                  Joan Bruna and
                  Dumitru Erhan and
                  Ian J. Goodfellow and
                  Rob Fergus},
  editor       = {Yoshua Bengio and
                  Yann LeCun},
  title        = {Intriguing properties of neural networks},
  booktitle    = {2nd International Conference on Learning Representations, 
                 {ICLR} 2014,
                  Banff, AB, Canada, April 14-16, 2014, Conference Track Proceedings},
  year         = {2014},
}

@book{kaczynski2004computational,
  title={Computational homology},
  author={Kaczynski, Tomasz and Mischaikow, Konstantin Michael and Mrozek, Marian},
  volume={157},
  year={2004},
  publisher={Springer}
}

 @book{dubrovin2012modern,
  title={Modern geometry—methods and applications: Part II: The geometry and topology of manifolds},
  author={Dubrovin, B. A. and Fomenko, A. T. and Novikov, S. P.},
  volume={104},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@inproceedings{DBLP:journals/corr/BurdaGS15,
  author       = {Yuri Burda and
                  Roger B. Grosse and
                  Ruslan Salakhutdinov},
  editor       = {Yoshua Bengio and
                  Yann LeCun},
  title        = {Importance Weighted Autoencoders},
  booktitle    = {4th International Conference on Learning Representations, {ICLR} 2016,
                  San Juan, Puerto Rico, May 2-4, 2016, Conference Track Proceedings},
  year         = {2016},
  url          = {http://arxiv.org/abs/1509.00519},
  timestamp    = {Thu, 25 Jul 2019 14:25:37 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/BurdaGS15.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}
